Projective Splitting with Forward Steps: Asynchronous and Block-Iterative Operator Splitting

This work is concerned with the classical problem of finding a zero of a sum of maximal monotone operators. For the projective splitting framework recently proposed by Combettes and Eckstein, we show how to replace the fundamental subproblem calculation using a backward step with one based on two forward steps. The resulting algorithms have the same kind of coordination procedure and can be implemented in the same block-iterative and highly flexible manner, but may perform backward steps on some operators and forward steps on others. Prior algorithms in the projective splitting family have used only backward steps. Forward steps can be used for any Lipschitz-continuous operators provided the stepsize is bounded by the inverse of the Lipschitz constant. If the Lipschitz constant is unknown, a simple backtracking linesearch procedure may be used. For affine operators, the stepsize can be chosen adaptively without knowledge of the Lipschitz constant and without any additional forward steps. We close the paper by empirically studying the performance of several kinds of splitting algorithms on a large-scale rare feature selection problem.

==> lassoNew-r1.tex <==
%!TEX root = forwProjMP-R1.tex
\section{Prelimary Numerical Experiments}
\label{secNumerical}
\subsection{Overview}
We now present some preliminary numerical experiments with \col{serial} variants of
Algorithm~\ref{AlgfullyAsync}.  \col{That is, we assume no delays so that $d(i,k)=k$. We do consider different block-iterative strategies for selecting $I_k$, as well as different cardinalities $|I_k|$.}
%Due to the extensive effort required to build and test an efficient highly parallel implementation, our experiments are based on a prototype serial implementation and do not reflect true parallelism or asynchronicity; however, we do try to assess the likely impact of asynchronicity delays and of imposing block structure like~\eqref{probCompMonoMany} onto superficially more monolithic problems.

%\subsection{$\ell_1$-regularized Least Squares}
A ubiquitous optimization problem with a plethora of currently popular applications is
$\ell_1$-regularized least squares, or lasso.
% This problem is typically used in machine learning/statistics under the guise
% of the lasso as well as in signal/image processing and compressed sensing.
We consider the problem
\begin{eqnarray}\label{probLasso}
\min_{x\in\mathbb{R}^d}
\left\{
\frac{1}{2}\|Qx - b\|_2^2
+
\lambda \|x\|_1
\right\},
\end{eqnarray}
where $Q\in\mathbb{R}^{m\times d}$, $b\in\mathbb{R}^m$, and $\lambda\geq 0$.
In the experiments we present here, we split problem~\eqref{probLasso} in the
following way: let $\calR = \{R_1,..,R_r\}$ be an arbitrary 
%% JE "partition" implies nonoverlapping
%nonoverlapping 
partition of
$\{1,\ldots,m\}$. For $i=1,\ldots,r$, let $Q_i\in\mathbb{R}^{|R_i|\times d}$
be the submatrix of $Q$ with rows corresponding to indices in $R_i$ and
similarly let $b_i\in\mathbb{R}^{|R_i|}$ be the corresponding subvector of
$b$.  Then a problem equivalent to~\eqref{probLasso} is
\begin{eqnarray}
\nonumber
%\label{probLassoSplit}
\min_{x\in\mathbb{R}^d}
\left\{
\frac{1}{2}
\sum_{i=1}^r
\|Q_i x - b_i\|_2^2
+
\lambda \|x\|_1
\right\},
\end{eqnarray} 
which is in the form of problem~\eqref{ProbOpt} and satisfies the constraint
qualification of \cite[Theorem 16.47(i)]{bauschke2011convex}.  Therefore, it
is a special case of \eqref{probCompMonoMany} with $n=r+1$, $G_i=I$
for $i=1,\ldots,r+1$,  $T_{i}(x)=Q_i^\top(Q_i x - b_i)$ for $i=1,\ldots,r$,
and $T_{r+1}(x) = \partial\{\lambda\|x\|_1\}$.  It is also possible to
consider a formulation in which the elements of $\calR$ overlap, but for
simplicity we do not consider this situation here. 
%In a distributed-memory parallel implementation, one may imagine that the block matrices $Q_i$ could be stored in different processors.

%  JE this is kind of speculative; best to leave such consideration until
%  later when we have a real parallel implementation.

% We have introduced the partition $\calR$ and corresponding submatrices $Q_i$
% so that if $Q$ is a huge matrix it is possible to store each $Q_i$ in a
% different processor memory. Alternatively, the data may be stored across
% machines for some other reason, such as security or privacy. Although we don't
% consider it here, it is also simple to accomodate overlapping partitions.
% Within the framework of Algorithm \ref{AlgfullyAsync}, all the data required
% for computation on each machine is given in $Q_i$ and no other parts of the
% data matrix are required.  As such, our algorithm can tackle problems where
% $Q$ exceeds the memory capacity of a single machine. We will assume that a
% central processor can communicate with each of these machines and is tasked
% with the projection calculations from Lines
% \ref{lineCoordStart}--\ref{eqAlgproj2}. This requires communicating copies of
% $(x_i^k,y_i^k)$ and $(z^k,w_i^k)$. This coordination phase is asynchronous
% making it much easier to implement and may also lead to large speed benefits
% as you avoid the need for ``locking", i.e. synchronizing the computations of
% all the processors (see \cite{hannah2017more} for examples where asynchrony
% leads to large benefits). On the implementation side we would expect $|R|$ to
% typically be between $10$ and $1000$ depending on the number of available
% computers in the cluster.

There are other possible ways to model problem~\eqref{probLasso} in the
form~\eqref{probCompMonoMany}: for example, one could set $G_i = Q_i$ and
$T_i(t) = \frac{1}{2}\|t - b_i\|^2$ for $i=1,\ldots,r$.  We will consider such
formulations in future work.

%%  JE thought this was way too long for something we are not doing.  Just substituted
%%  the very short paragraph above.

% Another approach to tackling Prob.~(\ref{probLassoSplit}) via Algorithm
% \ref{AlgfullyAsync} would be to extricate the linear operators from the
% containing Lipschitz differentiable functions. This could be done by setting
% $G_{i} = Q_i$ for $i=1,\ldots ,|R|$. This approach has two advantages. First
% it makes the stepsize constraints easy to satisfy as the operators are $T_{i}
% = \frac{1}{2}\|t - b_i\|^2$ which have Lipschitz constants equal to $1$.
% Second it also typically has a small memory footprint. The total memory
% complexity is $2d +2m$ variables whereas, as we will show below, the original
% approach stores $(2|R|+1)d$ variables  which is worse when
% $m<\frac{1}{2}(2|R|-1)d$.  The main disadvantage of extracting the linear
% operators is it cannot be implemented asynchronously. This is because lines
% \ref{lineCoordStart} and \ref{lineCoordEnd} of Algorithm \ref{AlgfullyAsync}
% compute $G_i x_{n}^k$ and $G_i^* w_{i}^k$ for $i=1,\ldots,|R|$ using the most
% up-to-date $w_{i}^k$ and $x_{n}^k$ possessed by the central processor. To do
% this either requires that the central processor has access to every $G_i$, or
% that it waits for each node with access to $G_i$ to provide this calculation,
% which would require synchronization. It may be possible to avoid the
% synchronization requirement however this analysis is left for future work.
% Nevertheless this approach does result in an interesting formulation which we
% plan to study in the future. For now in our current formulation each $G_i$ is
% the identity and the coordination done by the central processor does not need
% access to $Q$.

% In our testing, we set $\Ifor = \{1,\ldots,r\}$ and $\Iback = \{r+1\}$, that
% is, we use forward steps on the Lipschitz operators $T_1,\ldots,T_r$ and
% backward steps on the non-Lipschitz, multivalued operator $T_n = T_{r+1}$. 

% The function $\lambda_1\|\cdot\|_1$ corresponding to $T_n$ has a
% computationally simple proximal operator, 

The operator $T_n$ is not Lipschitz, so we always use backward steps to
process it.  The backward step for this operator is the well-known shrinkage
and soft thresholding operation, whose calculations are very simple and take
time linear in $d$.  Because of its simplicity, we process the operator $T_n$
at every iteration, that is, $n \in I_k$ for all $k \geq 1$.
%; in a distributed implementation, processing of $T_n$ could be considered as essentially part of the coordination process. 
Furthermore note that the entire
projection process conducted at each iteration from lines
\ref{lineCoordStart}-\ref{lineCoordEnd} of Algorithm~\ref{AlgfullyAsync}, has
$\bigO(d)$ computational complexity, and it remains $\bigO(d)$ even if we include
the processing of $T_n$ at every step.

On the other hand, the operators $T_i = Q_i^{\top}(Q_i(\cdot) - b_i)$, $i =
1,\ldots, r = n-1$, are Lipschitz and could be processed by either forward or
backward steps.  Since they are affine, we can furthermore use the stepsize
rule in Section~\ref{secOptStep}, which only requires two forward
steps per iteration, that is, two multiplies by $Q_i$ and two by $Q_i^\top$. We do
not need to estimate the largest eigenvalue of $Q$ or $Q_i$, a potentially
costly computation. 
%The optimized stepsize \eqref{eqOptimalStep} of Section~\ref{secOptStep} could also be used. In practice we found its performance to be very similar to that of~\eqref{eqAutoStepMod}, {}so for simplicity we only report results for the stepsize~\eqref{eqAutoStepMod}.
We will refer to the approach of setting $\Iforw = \{1,\ldots,r\}$ and using
the stepsize
rule from Section~\ref{secOptStep} as ``Projective Splitting with Forward
Steps'' (PSFor).
 
On the other hand, we could also process $T_1,\ldots,T_r$ with backward steps.
The corresponding proximal map is
\begin{eqnarray}\label{eqproxCongG}
\prox_{\rho \nabla\{\frac{1}{2}\|Q_i(\cdot) - b_i\|_2^2\}}(t)
=
(I+\rho Q_i^\top Q_i)^{-1}(t+\rho_i b).
\end{eqnarray}
A standard way to approach this calculation is to employ a matrix factorization
to solve the system of equations $(I + \rho Q_i^\top Q_i) x = t + \rho b$.  If
$\lvert R_i \rvert < d$, it may be preferable to use the matrix inversion lemma
as in~\cite{boyd2011distributed} to factor a matrix of dimension $\lvert R_i
\rvert \times \lvert R_i \rvert$ instead of the $d
\times d$ dimensional matrix $I + \rho Q_i^\top Q_i$.  But if both $d$ and
$\lvert R_i \rvert$ are large, then neither of these options may be attractive.  

Another option is to use an iterative solver to compute~\eqref{eqproxCongG};
this option is particularly attractive since our method tolerates errors in the
computation of backward steps.  So, we choose some $\sigma\in[0,1)$ and apply a
standard conjugate gradient algorithm to the linear system of equations
$(I + \rho Q_i^\top
Q_i) x = t + \rho b$ until the relative error criteria~\eqref{err1}
and~\eqref{err2} are met.

For a given candidate solution $x_{i}^k$, we have $y_{i}^k = Q_{i}^\top (Q_{i} x^k_i -
b_{i})$, and the error can be explicitly computed as $e_{i}^k = x^k_{i}
+\rho_{i} y^k_{i} -(z^{k}+\rho_{i} w_{i}^{k})$.  Every iteration of the
conjugate gradient algorithm requires two matrix multiplies, one by $Q_{i}$ and one by $Q_{i}^\top$. We ``warm-start" the conjugate gradient algorithm by
initializing it at $x^{k-1}_i$. We will refer to this approach as ``Projective
Splitting with Backward Steps'' (PSBack).

We compared PSFor and PSBack with two more established methods: FISTA
\cite{beck2009fast} and the relative error inexact version of ADMM proposed in
\cite[Algorithm~4]{eckstein2017relative}, which we will call RE-ADMM. For
FISTA, we used the backtracking linesearch variant. For RE-ADMM, we
experimented with different values for the relative error constant $\sigma$
and found $\sigma=0.9$ typically worked best for our test datasets. The
stepsize $c$ had to be tuned for each dataset and its values are given in
Table \ref{table_steps}.

To compare the methods fairly, we counted each algorithm's number of
``$Q$-equivalent" matrix multiplies --- multiplication by a matrix the size of
$Q$ or $Q^\top$. In applications with large data matrices, matrix
multiplications should be the dominant computation at each iteration. For
Algorithm \ref{AlgfullyAsync}, the number of ``$Q$-equivalent" multiplies
depends on the number of blocks $i\in I_k$ at each iteration and the size of
each block, corresponding to the number of rows in each matrix $Q_i$. Note
that $Q_i$ is a smaller matrix than $Q$, which we take into account as
follows: since $Q_i$ has $|R_i|$ rows and all the matrices in our testing are
dense, one $Q_i$ multiply counts as $|R_i|/m$ $Q$-equivalent multiplies.

We implemented  PSFor and PSBack in Python using the
\texttt{numpy} package.  
%Our present implementation is strictly serial, but able to simulate some asynchronous and block-iterative effects. 
We ran the algorithm with various values of $r$ with each block chosen to have the same
number of rows (or nearly so when $m$ is not divisible by $r$). At each
iteration, we selected one block from among $1,\ldots,r=n-1$ for a forward
step in PSFor or backward step with CG in PSBack, and block $n=r+1$ for a backward step.  Thus, $I_k$ always has the form $\{i,n\}$, with $1 \leq i < n$. To select this $i$, we tested the greedy block
selection scheme described in Section~\ref{secGreed}, as well as choosing
blocks at random. For the greedy scheme, we did not use the safeguard
parameter $M$ as in practice we found that every block was updated fairly
regularly. 
%We also considered various values for the maximum delay $D$ as defined in Assumption~\ref{assAsync}: for each activated block we simulated asynchonicity by uniformly randomly generating a delay $d(i,k)\in\{k-D,..,k\}$ while ensuring that the point $(w_i^{d(i,k)},z^{d(i,k)})$ used is newer than the last point used for that block.

%In this way we simulate an asynchronous computer cluster. 

\subsection{Experimental Details}

We considered three real datasets taken from the UCI Machine Learning
Repository \cite{Dua:2017}, as well as one synthetic dataset.  All the data
matrices were dense and we normalized their columns to have unit norm. The
datasets consisted of the gene expression cancer RNA-Seq 
dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/gene+expression+cancer+RNA-Seq}}
\cite{weinstein2013cancer} of size $3204\times 20531$, which we will refer to
as ``\emph{gene}", the ``\emph{drivFace}"
dataset\footnote{\url{https://archive.ics.uci.edu/ml/datasets/DrivFace}}
\cite{diaz2016reduced} of size $606\times 6400$, the sEMG hand gesture data 
set\footnote{\url{https://archive.ics.uci.edu/ml/datasets/sEMG+for+Basic+Hand+movements}.
We combined all $5$ subjects into one
dataset.}, \cite{sapsanis2013improving} of size $1800\times 3000$, which we
refer to as ``\emph{hand}", and finally a synthetic dataset of size
$1000\times 10000$ with all entries of $A$ and $b$ drawn i.i.d.
$\mathcal{N}(0,1)$. For \emph{gene}, the original dataset has $801$ examples.
We augmented each example with three ``noisy" copies, each being equal to the
original feature vector plus an i.i.d. zero-mean Gaussian random vector with
standard deviation equal to $0.1$ times the original population standard deviation.

For PSFor we used $\Delta=1$ and for PSBack we used $\sigma=0.9$ for all experiments. 
For the forward steps, instead of \eqref{eqAutoStep}, we used the modified 
rule
\begin{align}
\rho_i^k =
\min\left\{
\frac{\tilde{\rho}_i^k}{2}
,
\rho_i^{s(i,k-1)}
\right\},\quad i=1,\ldots,r,\quad k \geq 1,
\label{eqAutoStepMod2}
 \end{align}
which performed in a more stable manner in our experiments; recall that
$\rho_i^{s(i,k-1)}$ is the most recently used stepsize for the operator $T_i$.
To handle the case $k=1$, we set $\rho_i^0 = +\infty$. 

To set $\rho_{r+1}^k$ for PSFor, we used a heuristic inspired by the forward-backward method.  Specifically, we set
$\rho_{r+1}^{k}$ to be the average of the most recently used stepsizes across
all $i\in\Iforw$, that is, $\rho_{r+1}^{k} =
\frac{1}{r}\sum_{i=1}^r\rho_i^{s(i,k)}$. (If an operator has not yet been
updated with a forward step then it is not included in the average).

Table \ref{table_steps} displays the chosen values for $\gamma$ (which were
the same for PSFor and PSBack), the stepsizes for PSBack, and the parameter
$c$ for RE-ADMM.  For simplicity, the stepsizes in PSBack were fixed across
iterations. These parameters were chosen by running the algorithms for a small
number of iterations using a small selection of candidate values and seeing
which one worked best. The table also shows the model paramater $\lambda$,
which in each case was chosen so that the solution had approximately $10$\% of
its entries nonzero.

\begin{table}[h]
	\begin{center}
		
		\begin{tabular}{|l|r|r|r|r|r|}
			\hline 
			&gene&drivFace&hand&random\\
			\hline \hline
			$\gamma$&$100$&$100$&$1$&$1$
			\\
			\hline 
			$\rho_{1}\ldots\rho_{r}$ (PSBack)&$10^{-3}$&$1$&$0.1$&$0.1$
			\\
			\hline 
			$\rho_{r+1}$ (PSBack) &$10^{-3}$&$1$&$0.1$&$0.1$
			\\
			\hline    			
			$c$ (RE-ADMM) &$100$&$10$&$1$&$1$
			\\
			\hline     
			$\lambda$ &$10$&$10$&$1$&$1$
			\\
			\hline     
		\end{tabular}
	\end{center}
	\vspace{-2ex}
	\caption{Parameter settings for PSFor, PSBack, and RE-ADMM for the four lasso datasets\label{table_steps}.}	
\end{table}

Let $F(x)$ be the lasso objective defined in \eqref{probLasso}. We test the algorithms by comparing:
\begin{enumerate}
	\item the objective function residual: $(F(x_{alg}^m)-F^*)/F^*$, and
	\item the subgradient residual:
	$
	\min \{\|g\|: g\in\partial F(x_{alg}^m)\},
	$
\end{enumerate}
where $x_{alg}^m$ is an appropriate output iterate from each algorithm,  $F^*$
is the optimal value of the problem estimated by running all algorithms for
$10^5$ iterations and taking the minimum objective value, and $m$ counts the
number of ``$Q$-equivalent multiplies". For PSFor and PSBack,
$x_{alg}^m=x_{r+1}^m$, and for RE-ADMM $x_{alg}^m=z^m$ computed on the 
second-to-last line of \cite[Algorithm 4]{eckstein2017relative}.

In the subsequent results section we will use the following notation: \col{ 
PSFor$(r,R)$ means PSFor with $r$ blocks and with the active block randomly chosen at each iteration, and
similarly for PSBack$(r,R)$. PSFor$(r,G)$ means PSFor with $r$ blocks and the
greedy block selection strategy of Section \ref{secGreed}. If $r=1$ block is used, then we simply write PSFor$(1)$.}

\subsection{Results}

PSFor$(10,G)$ and PSBack$(10,G)$ were the best-performing variants of PSFor
and PSBack, respectively.  Figure~\ref{FigAll} compares these two algorithms with
FISTA and RE-ADMM on each of the four datasets. On all datasets except
\emph{drivFace}, PSFor$(10,G)$ performs the best. PSFor outperforms PSBack on all
datasets. 
\col{ 
Figure \ref{FigDelay} plots the improvement gained by using greedy block
selection instead of random block selection. The figure also demostrates that
PSFor$(1)$ is far slower than either variant with $10$ blocks.
 These results run counter to the typical behavior of decomposition
methods in optimization, which tend to converge more slowly the more
subsystems they must coordinate. Apparently, the reduced work per iteration
from the block-iterative implementation more than compensates for any
convergence slowdown resulting from generating new cut information from only
part of the problem at each step.}

%Figure \ref{FigDelay} plots the effect of increasing delay on PSFor and of not using the greedy block selection strategy. Both of these
%adversely effect the performance of the algorithm, but the degradation is
%fairly graceful. In a distributed setting this mild degradation may be
%outweighed by the considerable advantages and speedups offered by an
%asynchronous implementation. 

\begin{figure}
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugmentedfuncAll.pdf}	
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugmentedSGAll.pdf}	
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handfuncAll.pdf}	
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handSGAll.pdf}	
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFacefuncAll.pdf}	
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFaceSGAll.pdf}	
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomfuncAll.pdf}	
\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomSGAll.pdf}
\caption{Results on the four datasets. The left column plots function values in terms of relative error and the right column plots the minimum subgradient norm.}\label{FigAll}
\end{figure}

\begin{figure}
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugmentedfuncDelay.pdf}	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugmentedSGDelay.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handfuncDelay.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handSGDelay.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFacefuncDelay.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFaceSGDelay.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomfuncDelay.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomSGDelay.pdf}
	\caption{\col{Benefits of greedy block selection for PSFor. The left column plots function values in terms of relative error and the right column plots the minimum subgradient norm.}}\label{FigDelay}
\end{figure}

\subsection{Further Experiments: Blocks Processed Per Iteration}
In the previous experiments, the set of blocks to be processed at each
iteration was $I_k = \{i,r+1\}$, where $i \in \{1,\ldots,r\}$ was selected
either at random or by the greedy procedure of Section~\ref{secGreed}.  We now
consider the effect of choosing more than one least-squares block per
iteration, that is, setting $I_k = \{i_1,i_2,\ldots,i_b,r+1\}$ where
$\{i_j\}_{j=1}^b$ may be selected randomly or taken to be the ``best'' $b$
blocks according to the greedy criterion. We refer to these variants as
PSFor$(r,R,b)$ and PSFor$(r,G,b)$.  

Increasing $b$ increases the per-iteration complexity of the algorithm in a
straightforward way. Processing a block via forward steps requires two
multiplies by $Q_i$ and two by $Q_i^\top$. Hence, each additional block
requires $\bigO(md/r)$ more flops per iteration.

Figures \ref{FigOPIG} and \ref{FigOPIRandom} respectively show results for
PSFor$(10,G,b)$ and PSFor$(10,R,b)$, with $b=1,2,4,8$. Note that the $x$-axis
is now the number of iterations of Algorithm \ref{AlgfullyAsync}, not the
number of $Q$-equivalent multiplies. Rather suprisingly, PSFor$(10,G,1)$
performs almost as well as PSFor$(10,G,b)$ for $b=2,4,8$, even though it only
processes one block per iteration and hence has far lower per-iteration
complexity. It seems that most of the information required to create a ``good"
separating hyperplane is contained in just one block. For randomly chosen
blocks, there is greater benefit to using more than one block, especially
for the \emph{random} and \emph{gene} datasets.  However, on the \emph{hand} and \emph{drivFace} datasets there is
little benefit.  In all experiments there is little or no advantage to employing
more than two blocks per iteration.

These experiments suggest that processing many blocks per iteration
may well be undesirable. A similar convergence rate can be achieved with much lower
per-iteration complexity by processing just one or two blocks per iteration,
expecially if using the greedy selection criterion.

%MP version
%\begin{acknowledgements}
%This material is based upon work supported by the National Science 
%Foundation under Grant No. 1617617.
%\end{acknowledgements}



\begin{figure}
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugfuncOPIGreedy.pdf}	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugSGOPIGreedy.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handfuncOPIGreedy.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handSGOPIGreedy.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFacefuncOPIGreedy.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFaceSGOPIGreedy.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomfuncOPIGreedy.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomSGOPIGreedy.pdf}
	\caption{Effect of the number of blocks processed per iteration with greedy block selection. The left column plots function values in terms of relative error and the right column plots the minimum subgradient norm.}\label{FigOPIG}
\end{figure}
\begin{figure}
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugfuncOPIRandom.pdf}	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/geneAugSGOPIRandom.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handfuncOPIRandom.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/handSGOPIRandom.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFacefuncOPIRandom.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/drivFaceSGOPIRandom.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomfuncOPIRandom.pdf}	
	\includegraphics[width=0.5\textwidth,height=5cm]{Figs/randomSGOPIRandom.pdf}
	\caption{Effect of the number of blocks processed per iteration with random block selection. The left column plots function values in terms of relative error and the right column plots the minimum subgradient norm.}\label{FigOPIRandom}
\end{figure}








==> old_async_sec.tex <==
One simple option is a centralized or ``master-slave'' implementation in which lines~\ref{lineaupdate}-\ref{lineBackwardUpdateY} and~\ref{ForwardxUpdate}-\ref{ForwardyUpdate} are implemented on a collection of ``worker'' processors, while the remainder of the algorithm, most notably the coordination process embodied by lines~\ref{lineCoordStart}-\ref{lineCoordEnd}, is executed by a single coordinating processor.  However, such a simple implementation risks the coordinating processor becoming a serial bottleneck as the number of worker
processors grows or the memory required to store the vectors
$(x_i^k,y_i^k,w_i^k)$ for $i = 1,\ldots,n$, becomes large, since the amount of
work required to execute lines~\ref{lineCoordStart}-\ref{lineCoordEnd} is
proportional to the total number of elements in $(x_i^k,y_i^k,w_i^k)$.
Fortunately, all but a constant amount of the work in the coordination
calculations in lines~\ref{lineCoordStart}-\ref{lineCoordEnd} involves only
sums, inner products, and matrix multiplies by $G_i$ and $G_i^*$.  Summation
and hence inner product operations can be efficiently distributed over
multiple processors.  Therefore, with some care exercised as to where one
performs the matrix multiplications in cases in which the $G_i$ are
nontrivial, the coordination calculations may be distributed over multiple
processors so that the coordination process need not constitute a serial
bottleneck.

==> old_async_two.tex <==
In the simple ``master-slave'' scheme
described above, for example, the ``master'' might dispatch subproblems to
worker processors, but not receive the results back immediately.  In the
meantime, other workers may report back results, which the master could
incorporate into its projection calculations.  In this context, $k$ counts the
number of projection operations performed at the master, and $I_k$ is the set
 of subproblems whose solutions reached the master between iterations
$k-1$ and $k$.  For each $i \in I_k$, $d(i,k)$ is the index of the iteration
completed just before subproblem was last dispatched for solution.  In more
sophisticated parallel implementation, $I_k$ and $d(i,k)$ would have similar
interpretations.
